Horizontal spreading of planetary debris accreted by white dwarfs

White dwarfs with metal-polluted atmospheres have been studied widely in the context of the accretion of rocky debris from evolved planetary systems. One open question is the geometry of accretion and how material arrives and mixes in the white dwarf surface layers. Using the 3D radiation-hydrodynamics code CO$^5$BOLD, we present the first transport coefficients in degenerate star atmospheres which describe the advection-diffusion of a passive scalar across the surface-plane. We couple newly derived horizontal diffusion coefficients with previously published vertical diffusion coefficients to provide theoretical constraints on surface spreading of metals in white dwarfs. Our grid of 3D simulations probes the vast majority of the parameter space of convective white dwarfs, with pure-hydrogen atmospheres in the effective temperature range 6000-18000 K and pure-helium atmospheres in the range 12000-34000 K. Our results suggest that warm hydrogen-rich atmospheres (DA; $\gtrsim$13000 K) and helium-rich atmospheres (DB, DBA; $\gtrsim$30000 K) are unable to efficiently spread the accreted metals across their surface, regardless of the time dependence of accretion. This result may be at odds with the current non-detection of surface abundance variations at white dwarfs with debris discs. For cooler hydrogen- and helium-rich atmospheres, we predict a largely homogeneous distribution of metals across the surface within a vertical diffusion timescale. This is typically less than 0.1 per cent of disc lifetime estimates, a quantity which is revisited in this paper using the overshoot results. These results have relevance for studies of the bulk composition of evolved planetary systems and models of accretion disc physics.

==> Horizontal Mixing/table2-3-merged.tex <==
\begin{table*}
	\centering
        \caption{Diffusion coefficients defined by Eq.~\eqref{eq:Dreal} for pure-hydrogen DA white dwarf atmospheres. Computed using mean 3D quantities from a grid of cool DAs ($\leqslant13\,000$\,K) from \citet{tremblay13a}, except for those with $11\,600\,\mathrm{K}\leqslant T_{\rm eff}\leqslant 18\,000$\,K and $\log g=8.0$, which were computed using the grid of deep simulations from \citetalias{cunningham19}. \change{The simulations leading to the results in this table utilised a non-grey opacity scheme for the radiative transfer}. We also show the upper limit on the diffusion coefficient (corresponding to the photospheric layers) defined by Eq.~\eqref{eq:Dgran}. The real effective temperature of a simulation can stabilise at a slightly different \change{effective temperature} to the desired value. To represent this we include the quantity $\Delta(T)$ such that the true effective temperature is given by $T_{\rm eff} + \Delta(T)$. An explicit error is not available for these results, but we note that typical \change{statistical} errors from the direct diffusion experiments (Table~\ref{tb:D3d}) were on the order of $\sigma(\log \mDhor)\approx0.1$. \change{An additional source of uncertainty arises in Fig.\,\ref{fg:direct_full} from the imperfect fit of the directly derived diffusion coefficients to those computed from physical parameters. We find at the warmest end of the grid the difference is as large as 0.2 and 0.4 dex for \Dhor\ and \Dhormax, respectively.}
%        	\change{An additional source of uncertainty arises from the difference between diffusion coefficients derived for grey models (Table\,\ref{tb:D3d}) and those derived from the non-grey models presented in this table. For most simulations this discrepancy is on the order of the statistical uncertainty ($\sim$0.1 dex). For simulations with effective temperatures 13\,500--16\,000\,K we find the difference in $D_{\rm surf}$ and $D_{\rm surf}^{\rm max}$ computed from grey and non-grey models to be on the order of $\sim$0.2--0.5\,dex.}
    }
%        \label{tab:}
        \begin{tabular}{lclcccclclcc}
                 \cline{1-5} \cline{8-12}
                 \vspace{5pt}
$T_{\rm eff}$  & $\log g$ & $\Delta(T)$ & $\log$ \Dhor & $\log$ \Dhormax &   &   & $T_{\rm eff}$  & $\log g$ & $\Delta(T)$ & $\log$ \Dhor & $\log$ \Dhormax \Tstrut \\
%\vspace{5pt}
$\mathrm{[K]}$  & [cm\,s$^{-2}$] & [K] & [cm$^{2}$\,s$^{-1}$] & [cm$^{2}$\,s$^{-1}$] &   &   & $\mathrm{[K]}$  & [cm\,s$^{-2}$] & [K] & [cm$^{2}$\,s$^{-1}$] & [cm$^{2}$\,s$^{-1}$] \Bstrut\\
				
                \cline{1-5} \cline{8-12}
               
                 7000  &   7.00 &  +46 &   9.38 &   9.88 &   &   &    13000  &   8.00 &   +4 &   9.31 &   9.97 \Tstrut\\
                8000  &   7.00 &  +27 &   9.63 &  10.19 &   &   &    13500  &   8.00 &   +1 &   9.25 &   9.84 \\ 
                9000  &   7.00 &  +25 &   9.88 &  10.47 &   &   &    14000  &   8.00 &   +1 &   9.09 &   9.65 \\ 
                9500  &   7.00 &  +21 &  10.03 &  10.64 &   &   &    14500  &   8.00 &   -2 &   8.89 &   9.41 \\ 
                10000  &   7.00 &  +18 &  10.25 &  10.88 &   &   &    15000  &   8.00 &   +0 &   8.66 &   9.16 \\ 
                10500  &   7.00 &  +40 &  10.45 &  11.13 &   &   &    15500  &   8.00 &   +1 &   8.32 &   8.81 \\ 
                11000  &   7.00 &   +0 &  10.40 &  11.09 &   &   &    16000  &   8.00 &   +2 &   7.99 &   8.50 \\ 
                11500  &   7.00 &   +1 &  10.24 &  10.80 &   &   &    16500  &   8.00 &   +3 &   7.06 &   7.54 \\ 
                12000  &   7.00 &   +1 &  10.14 &  10.64 &   &   &    17000  &   8.00 &   +3 &   6.55 &   7.44 \\ 
                12500  &   7.00 &   +1 &   9.93 &  10.40 &   &   &    17500  &   8.00 &  +24 &   5.78 &   7.02 \\ \vspace{5pt}  
                13000  &   7.00 &   +3 &   9.79 &  10.30 &   &   &    18000  &   8.00 &  +21 &   5.35 &   6.61 \\ 
                6000  &   7.50 &  +65 &   8.42 &   8.83 &   &   &      6000  &   8.50 &  +24 &   7.13 &   7.61 \\ 
                7000  &   7.50 &  +33 &   8.78 &   9.22 &   &   &    7000  &   8.50 &  -75 &   7.68 &   8.13 \\ 
                8000  &   7.50 &  +17 &   9.02 &   9.55 &   &   &    8000  &   8.50 &   +4 &   7.79 &   8.28 \\ 
                9000  &   7.50 &  +15 &   9.24 &   9.84 &   &   &    9000  &   8.50 &  +68 &   8.02 &   8.58 \\ 
                9500  &   7.50 &  +49 &   9.37 &   9.98 &   &   &    9500  &   8.50 &  +22 &   8.11 &   8.68 \\ 
                10000  &   7.50 &   +7 &   9.53 &  10.15 &   &   &    10000  &   8.50 &  -28 &   8.20 &   8.80 \\ 
                10500  &   7.50 &   +0 &   9.71 &  10.37 &   &   &    10500  &   8.50 &   -4 &   8.32 &   8.95 \\ 
                11000  &   7.50 &  -62 &   9.87 &  10.39 &   &   &    11000  &   8.50 &   -3 &   8.44 &   9.09 \\ 
                11500  &   7.50 &   -2 &   9.95 &  10.70 &   &   &    11500  &   8.50 &  -10 &   8.58 &   9.24 \\ 
                12000  &   7.50 &   -1 &   9.87 &  10.55 &   &   &    12000  &   8.50 &  -21 &   8.72 &   9.41 \\ 
                12500  &   7.50 &   +0 &   9.76 &  10.32 &   &   &    12500  &   8.50 &  -80 &   8.88 &   9.60 \\ \vspace{5pt}
                13000  &   7.50 &   +2 &   9.67 &  10.18 &   &   &   13000  &   8.50 &  -91 &   8.97 &   9.74 \\
			     6000  &   8.00 &   -3 &   7.82 &   8.28 &   &   &    6000  &   9.00 &  +28 &   6.74 &   7.28 \\ 
			     7000  &   8.00 &  +11 &   8.16 &   8.60 &   &   &    7000  &   9.00 &  -40 &   6.99 &   7.45 \\ 
			     8000  &   8.00 &  +34 &   8.41 &   8.91 &   &   &    8000  &   9.00 &  +41 &   7.19 &   7.64 \\ 
			     9000  &   8.00 &  +36 &   8.63 &   9.22 &   &   &    9000  &   9.00 &   -1 &   7.41 &   7.93 \\ 
			     9500  &   8.00 &  +18 &   8.73 &   9.32 &   &   &    9500  &   9.00 &   +7 &   7.50 &   8.05 \\ 
			    10000  &   8.00 &  +25 &   8.85 &   9.46 &   &   &    10000  &   9.00 &  -38 &   7.58 &   8.16 \\ 
			    10500  &   8.00 &  +32 &   9.01 &   9.65 &   &   &    10500  &   9.00 &  -97 &   7.66 &   8.27 \\ 
			    11000  &   8.00 &   +5 &   9.15 &   9.81 &   &   &    11000  &   9.00 &  -52 &   7.78 &   8.41 \\ 
			    11500  &   8.00 &  +29 &   9.33 &  10.02 &   &   &    11500  &   9.00 &  -85 &   7.88 &   8.53 \\ 
			    11600  &   8.00 &  +41 &   9.37 &  10.09 &   &   &    12000  &   9.00 &  -85 &   8.01 &   8.68 \\ 
			    12000  &   8.00 &   +8 &   9.45 &  10.16 &   &   &    12500  &   9.00 &  -64 &   8.14 &   8.84 \\ 
			    12500  &   8.00 &   +9 &   9.42 &  10.16 &   &   &    13000  &   9.00 &  -31 &   8.28 &   9.02 \Bstrut\\
			    
%			    13000  &   8.00 &   +4 &   9.31 &   9.97 \\
%			    13500  &   8.00 &   +1 &   9.25 &   9.84 \\ 
%			    14000  &   8.00 &   +1 &   9.09 &   9.65 \\ 
%			    14500  &   8.00 &   -2 &   8.89 &   9.41 \\ 
%			    15000  &   8.00 &   +0 &   8.66 &   9.16 \\ 
%			    15500  &   8.00 &   +1 &   8.32 &   8.81 \\ 
%			    16000  &   8.00 &   +2 &   7.99 &   8.50 \\ 
%			    16500  &   8.00 &   +3 &   7.06 &   7.54 \\ 
%			    17000  &   8.00 &   +3 &   6.55 &   7.44 \\ 
%			    17500  &   8.00 &  +24 &   5.78 &   7.02 \\  \vspace{5pt}  
%			    18000  &   8.00 &  +21 &   5.35 &   6.61 \\ 
%                 6000  &   8.50 &  +24 &   7.13 &   7.61 \\ 
%			    7000  &   8.50 &  -75 &   7.68 &   8.13 \\ 
%			    8000  &   8.50 &   +4 &   7.79 &   8.28 \\ 
%			    9000  &   8.50 &  +68 &   8.02 &   8.58 \\ 
%			    9500  &   8.50 &  +22 &   8.11 &   8.68 \\ 
%			    10000  &   8.50 &  -28 &   8.20 &   8.80 \\ 
%			    10500  &   8.50 &   -4 &   8.32 &   8.95 \\ 
%			    11000  &   8.50 &   -3 &   8.44 &   9.09 \\ 
%			    11500  &   8.50 &  -10 &   8.58 &   9.24 \\ 
%			    12000  &   8.50 &  -21 &   8.72 &   9.41 \\ 
%			    12500  &   8.50 &  -80 &   8.88 &   9.60 \\ \vspace{5pt}
%			    13000  &   8.50 &  -91 &   8.97 &   9.74 \\
%			    6000  &   9.00 &  +28 &   6.74 &   7.28 \\ 
%			    7000  &   9.00 &  -40 &   6.99 &   7.45 \\ 
%			    8000  &   9.00 &  +41 &   7.19 &   7.64 \\ 
%			    9000  &   9.00 &   -1 &   7.41 &   7.93 \\ 
%			    9500  &   9.00 &   +7 &   7.50 &   8.05 \\ 
%			    10000  &   9.00 &  -38 &   7.58 &   8.16 \\ 
%			    10500  &   9.00 &  -97 &   7.66 &   8.27 \\ 
%			    11000  &   9.00 &  -52 &   7.78 &   8.41 \\ 
%			    11500  &   9.00 &  -85 &   7.88 &   8.53 \\ 
%			    12000  &   9.00 &  -85 &   8.01 &   8.68 \\ 
%			    12500  &   9.00 &  -64 &   8.14 &   8.84 \\ 
%			    13000  &   9.00 &  -31 &   8.28 &   9.02 \\
               \cline{1-5} \cline{8-12}
        \end{tabular}
        \label{tb:Dderived_DA_full}\\
\end{table*}


==> Horizontal Mixing/table4-cukanovaite19-new.tex <==
\begin{table}
	\centering
        \caption{Similar to Table~\ref{tb:Dderived_DA_full} for the grid of DB white dwarfs (log [H/He] = $-$10) from \citet{cukanovaite19}.}
        \label{tab:Dderived_DB}
        \begin{tabular}{lclcc}
                \hline            
                 \vspace{5pt}
$T_{\rm eff}$  & $\log g$ & $\Delta(T)$ & $\log$ \Dhor & $\log$ \Dhormax \\
%[K]  & [cm\,s$^{-2}$] & [K] & [cm$^{2}$\,s$^{-1}$] & [cm$^{2}$\,s$^{-1}$] \\
$\mathrm{[K]}$  & [cm\,s$^{-2}$] & [K] & [cm$^{2}$\,s$^{-1}$] & [cm$^{2}$\,s$^{-1}$] \\
\hline
12000  &   7.50 &  +98 &   8.10 &   8.47 \\
14000  &   7.50 &  -31 &   8.38 &   8.83 \\ 
16000  &   7.50 &  -53 &   8.65 &   9.19 \\ 
18000  &   7.50 &  +59 &   8.96 &   9.52 \\ 
20000  &   7.50 &  -69 &   9.41 &  10.09 \\ 
22000  &   7.50 &  +44 &   9.64 &  10.68 \\ 
24000  &   7.50 & -226 &   9.74 &  10.87 \\ 
26500  &   7.50 &   -3 &   9.83 &  10.93 \\ 
28000  &   7.50 &   -3 &   9.77 &  10.85 \\ 
30000  &   7.50 &   -7 &   9.63 &  10.65 \\ \vspace{5pt}
32000  &   7.50 &   +1 &   9.50 &  10.46 \\ 
12000  &   8.00 &  +20 &   7.42 &   7.75 \\ 
14000  &   8.00 &  +83 &   7.77 &   8.20 \\ 
16000  &   8.00 & +105 &   8.05 &   8.57 \\ 
18000  &   8.00 &  +82 &   8.32 &   8.89 \\ 
20000  &   8.00 &  +90 &   8.66 &   9.27 \\ 
22000  &   8.00 &   +5 &   9.06 &   9.88 \\ 
24000  &   8.00 & +144 &   9.18 &  10.23 \\ 
26000  &   8.00 & -102 &   9.25 &  10.35 \\ 
28000  &   8.00 & +107 &   9.32 &  10.39 \\ 
30000  &   8.00 &   -3 &   9.33 &  10.40 \\ 
32000  &   8.00 &   +1 &   9.30 &  10.30 \\ \vspace{5pt}
34000  &   8.00 &   +0 &   9.17 &  10.11 \\ 
12000  &   8.50 & +139 &   6.83 &   7.20 \\ 
14000  &   8.50 &   +7 &   7.15 &   7.55 \\ 
16000  &   8.50 &  -39 &   7.42 &   7.89 \\ 
18000  &   8.50 &   +0 &   7.68 &   8.23 \\ 
20000  &   8.50 &  -45 &   7.94 &   8.53 \\ 
22000  &   8.50 &   -1 &   8.33 &   9.00 \\ 
24000  &   8.50 & +143 &   8.61 &   9.53 \\ 
26000  &   8.50 & -195 &   8.67 &   9.72 \\ 
28000  &   8.50 &  -66 &   8.76 &   9.85 \\ 
30500  &   8.50 &  +67 &   8.88 &   9.95 \\ 
32000  &   8.50 & +208 &   8.88 &   9.94 \\ \vspace{5pt}
34000  &   8.50 &  +20 &   8.90 &   9.92 \\ 
12000  &   9.00 & +124 &   6.22 &   6.56 \\ 
14000  &   9.00 & +117 &   6.56 &   6.97 \\ 
16000  &   9.00 &  +29 &   6.82 &   7.28 \\ 
18000  &   9.00 &   -2 &   7.05 &   7.58 \\ 
19500  &   9.00 &  +31 &   7.25 &   7.84 \\ 
22000  &   9.00 &  -22 &   7.59 &   8.23 \\ 
24000  &   9.00 &  +82 &   7.95 &   8.71 \\ 
26000  &   9.00 & +116 &   8.10 &   9.03 \\ 
28000  &   9.00 & +143 &   8.19 &   9.23 \\ 
30000  &   9.00 & +184 &   8.27 &   9.33 \\ 
31500  &   9.00 &  -60 &   8.32 &   9.38 \\ 
34000  &   9.00 & +105 &   8.43 &   9.46 \\
                \hline
        \end{tabular}
        \label{tb:Dderived-DB}\\
\end{table}
